An Integrated P2P Framework for E-Learning

The paper is concerned with the design and development of a P2P Presentation System (P2P-PS) for live streaming of lectures coupled with a shareable whiteboard. Video streaming uses a data-driven modified mesh architecture which supports dynamic fanout. The whiteboard may be used in synchronization with an active video streaming session. It is shared by both the presenter and the participants in the audience for graphic illustrations during the lecture. P2P-PS provides an important feature called {\em ask doubt} that allows any participant to send a query (or a doubt) during an active presentation session. The query is disseminated to all other peers by preserving the causality between {\em ask doubt} and its resolution. A buffered approach is employed to boost the performance of the whiteboard. The simulations experiments were performed with over 1000 peer nodes on Emulab using 200 physical nodes. The results show that the proposed overlay eventually stabilizes even in the presence of a churning rate of up to 30\%. The maximum path length being just six hops. The estimated throughput is found to be close to our theoretical results.

==> modifiedMesh.tex <==
The fanout value cannot be arbitrary. It is determined by the upload bandwidth capacity and streaming rate. 
The fanout value determines the number of children a node may support. However, a node cannot support a faster outflow rate than its inflow rate. A relationship should exist between the in-degree and out-degree of a node for receiving the data packets continuously. We continue to abuse the terms "parent" and "children" of a node while referring respectively to a neighbor on an inflow path and a neighbor on an outflow path. 

Over the duration of an entire session, all nodes except for the ones connected directly to the source will have to maintain the relationship, 'in-degree $\leq$ out-degree'.  This does not preclude the relationship 'in-degree $>$ out-degree'. So, a node can have more number of inflow than the number of outflow. It essentially implies that a node have more parents than children. However, we discard such a case, because in this case a recipient gets more packets than it could send. Eventually such a node will run into a buffer overflow problem at the receiver side leading to loss of multiple packets and re-transmissions. 

We divide the media contents for streaming into chunks. These chunks are propagated to the peers where they could assemble them to a media file. The presenter is at the source node which streams the media contents to its neighboring peers. Being a multi-parent, multi-child architecture, a peer could ask for chunks from its parent peers and deliver these to its children. As stated earlier, whenever a source node joins the system, it authenticates itself from the bootstrap server. Once, it is authenticated, the presenter could start streaming data. However, it will not send data to any of its children unless explicitly asked. Whenever a new peer joins the system, it will get a list of nodes from the bootstrap server.  A set of parents will be assigned to the newly joined node. As soon as the node gets attached to its first parent, it will ask the parent about the latest (current) streaming packet id. Assume that a peer $P_x$  have parents $P_0$, $P_1, P_2, P_3, \ldots, P_k$. Let $P_x$ receive its latest packet information from parent $P_0$. Let the chunks ids are assigned in increasing or $id_0$, $id_1, id_2, id_3, id_4, \ldots$, and so on. Further let the latest packet be $id_0$. Hence, in round 1, peer $P$ will request for $id_0$ from $P_0$, $id_1$ from $P_1$, $id_2$ from $P_2$, and so on, $id_k$ from $P_k$. Suppose, $P_x$ gets initial reply from $P_3$, then from $P_1$, then from $P_k$, etc. So, peer $P_x$ will ask for $id_{k+1}$ from $P_3$, $id_{k+2}$ from $P_1$, $id_{k+3}$ from $P_k$ and so on. In other words, a peer will ask for the next id from the parent which replies first. This will create a stack of ids at the parent side. This process is done parallely.\\ 
The above procedure is depicted below:
Assume the following partial random mesh as shown in figure \ref{fig:Mesh}:
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{images/Mesh.png}
    \caption{Partial view of mesh overlay}
    \label{fig:Mesh}
\end{figure}
% {\bf Comment: Use a diagram to illustrate the concept}

Consider the node $P_x$ and its parent only. The request and reply for latest packet id is depicted in figure \ref{fig:Req}

\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{Req}
    \caption{Request and reply sequence for latest packet id}
    \label{fig:Req}
\end{figure}

Once id of latest packet is received, how the initial request for subsequent packet is made is shown in figure \ref{fig:preq}.
\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{preq}
    \caption{Initial request for packets}
    \label{fig:preq}
\end{figure}

The next packets requests are sent to the parent peers according to the order of their replies. Figure \ref{fig:subreq} provides further illustration.
\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{subreq}
    \caption{Request for subsequent packets}
    \label{fig:subreq}
\end{figure}

Whenever a packet is received from any of its parents, id should be updated such that request for next id could be placed.  Hence, id updating procedure is done in a mutually exclusive manner. It could be observed that request for id is sent to a parent even when the id is not available. It is like doing an advance reservation for a packet of a particular id. Also with this approach there is no need of any scheduling technique. It could be imagined as a peer is saying to its parent that whenever this particular id is available immediately send me so that I could make a reservation for subsequent ids. A peer also remembers about the ids which it has asked to its parents. At any point of time, a parent is asked to send only one packet. Hence, a peer needs to remember only about one packet id.

\section{Leaving of a Node}

Handling leaving of a node when it quits gracefully has been discussed earlier. Now we discuss how involuntary leaving of a peer is handled. We know that, at any point in time, a peer has to remember only about id which it has requested to its parents. Hence, if a parent fails abruptly, it will result in loss of only one chunk. Assume that it takes $x$ units of time for transferring a chunk between a sender and a receiver peer. That is $x$ is the delay between a request for a packet, and receiving the response. If a peer has asked for id from its parent, and there is no response for the $2\times x$ duration of time, then the peer compares the 'requested id' with id of the last packet it has received. If asked requested id is less than the last packet id it has received, then it is assumed that either the concerned node does not have that packet or it is not alive. So, it creates another request id for the same packet from some other peer. It implies that unavailability of one chunk may result in delay of $2\times x+x$=$3\times x$ time units. The missing chunk is recovered from other parent nodes. 

If a peer experience a delay of $\text{time out} = 2\times x$ units for any of the parent node, then that particular parent information is notified to the bootstrap server by the peer. Bootstrap server then explicitly initiates 'Are you alive?' message to that parent. Assume that it takes $y$ unit of time for sending message to a node, then it will wait for $2\times y$ units of time for reply. If there is no response, then it is safe to assume that, that a particular node is dead. In that case, the bootstrap server removes non responding node from the list of active peers list. The bootstrap server then informs the child node about the loss of his parent node so that it could update its parent list. We are storing the children list with its parent only. Hence, if a node exits involuntarily, then none of its children gets be any information about the parent's leaving. Every child node needs to figure out on its own about the failure of its parent. Suppose a node has only one parent left and that parent eventually fails involuntarily. In this situation the orphaned peer requests the bootstrap server to assign a new set of parents. This might incorporate some delay. To handle the case of orphaned node, we modified our approach a bit more. Once, a child notices that it has less than $\frac{k}{2}$ parents it requests the bootstrap server to allocate at least one more parent to it. The reason for choosing at least 1 is because of flash crowd. When the lecture is about to end, then lots of peers start leaving the system. Hence, there is high chance that count will fall below $\frac{k}{2}$ at a faster rate. Also, at that point it might not be possible to always satisfy the requirement of $k$ parents. In the worst case only a source node and a single peer may be available, and all other nodes have departed. In this case, source could be the only parent of the remaining peer. Hence, it will make more sense for that peer to ask from the bootstrap server for atleast one parent node. 
% {\bf Comment not clear}  

\section{Handling "Ask Doubt"}
Every peer is aware of the source node's address. Whenever a person wants to ask a doubt he/she clicks on 'ask doubt' button provided in UI of our application. This establishes a direct connection with the presenter. The presenter will see the 'ask doubt' request. Doubt message will be in the form of an audio message. If the presenter is free, i.e. if he/she is not answering any other doubts, then he/she will acknowledge the request. Only after receiving an acknowledgement, the requesting person is allowed to ask a doubt. The doubt, in the form of an audio message, will be directly propagated to the presenter first. It could be said that message is directly pushed on the link between them. Its child peers will then pull the video data. Hence, spreading of doubt will happen in a push-based manner as happens in tree based approach. This will guarantee that no question is answered before it is asked thereby preserving the causality relationship. 

\section{Memory Utilization}
Video packet consist of following information: Video data, start of data, length of data. We are maintaining a dictionary for storing packets called PList. PList will store recent $10\times1024$ packet data. Each packet size is 1400 bytes. Our streaming rate is 2 Mbps.\\Number of packets generated per second = $\frac{2\times10^6}{1400\times8}$ = 179 packets.\\ 
The maximum amount of video data that can reside in PList is $10\times1024\times1400\approx14MB$.\\
When size(PList)$>=10\times1024$, then for inserting new packet in the data list, oldest packet video data is removed from the PList \\
Video data available in PList could run a session for $\frac{10\times1024}{179}\approx 57$ seconds. 
\\Older data will be needed only if session exceeds this limit. Note that only video data is removed, start and length fields remains unchanged.\\
Consider the case where session is running for 8 continuous hours. \\
Number of packets generated in 8 hours = $179\times8\times60\times60$ packets.\\
Total memory consumed by PList in 8 hours = $179\times8\times60\times60\times(8+8)+1024\times10\times1400 \approx 100MB$

==> resultDebruijn.tex <==

\section{Experiments and Results}
\label{sec:experiments}

Emulab provides an environment for experiments over test beds consisting of large-scale distributed network. We deployed the scripts for the experiments using Emulab portal to acquire both physically distributed and purely simulated nodes~\cite{emulab2008}. It fitted the kind of experiments we wanted to run for establishing efficacy of our approach to build a low latency file sharing, searching and inline annotations framework ideally suitable for E-learning system using a P2P organization. 

As indicated in section~VI, the underlying de Bruijn graph has diameter and out-degree equal to eight. At the application layer, the diameter does not exceed the value of eight. But, out-degree can typically vary according to size of a zone. In theory, the maximum out-degree would be less than $K \times O(\log_K{N})$ with high probability. Here $N$ is the number of nodes in the system. Considering $N=800,000$ nodes, the maximum out-degree among all runs was 41. For every result of different values of $N$, the average out-degree was 7.99. The value of 7.99 is due to lack of self-loops. 
\begin{figure}%{l}{0.3\textwidth}
    \centering
    \includegraphics[scale=0.5]{images/UptoThousand.png}
    \caption{Maximum out-degree of nodes}
    \label{fig:upto-thousand}
\end{figure}
\begin{figure}%{l}{0.3\textwidth}
    \centering
    \includegraphics[scale=0.5]{images/UptoMillions.png}
    \caption{Maximum out-degree of nodes}
    \label{fig:upto-million}
\end{figure}
\begin{figure}%{l}{0.3\textwidth}
    \centering
    \includegraphics[scale=0.5]{images/Dist.png}
    \caption{Distribution graph of out-degree of nodes}
    \label{fig:key-distro}
\end{figure}

The graph in~\ref{fig:upto-thousand} and~\ref{fig:upto-million} show that the median values of the maximum out-degree of a node. The results from simulations match with the theoretical results. 
The graph shows that the median value for the maximum out-degree when $N=100000$ is 31. The distribution of out-degree for the same is shown in~\ref{fig:key-distro}. As may be found from the distribution, very few nodes have degree $> 2\times K$. Only 380 nodes out of 100000 have degree $> 16$, which is only $0.38\%$ of the nodes. None of the nodes have out-degree $> K \times \log\_K{100000}$. This is certainly much better than an equivalent Chord implementation, where average out-degree would be equivalent to $O(\log N)$ or more than 20.
The experiments also showed that, minimum in-degree was 7, and the maximum was 8. The minimum in-degree is 7 because edges of self-loops are not counted.

We also carried out experiments on Emulab to find out the maximum latency and the success rate of look-ups. In the experiment, the nodes were connected to each other in a LAN environment. Every node randomly picked twenty-five words from the list of three thousand words available to everyone. After a delay of five minutes, the nodes sent out queries for the same set of words. The boot-up times of machines provided by Emulab differ up to $\pm 5$ minutes. Hence, the join procedure for de Bruijn overlay network would have involved a transfer of the load for most of the nodes. The results were calculated for the different number of nodes as shown in Table~\ref{tab:exp1}. They indicate that none of the lookups failed, even during the dynamic joins in the set up.
\begin{table}[h!]
 \caption{Lookup latency and success rate}
    \label{tab:exp1}
    \begin{center}
     \begin{tabular}{||c | c | c | c||} 
     \hline
     \bf{No. of nodes} & \bf{Success rate} & \bf{Max Lat.(ms)} & \bf{Avg. Lat.(ms)}\\
     \hline\hline
    80 & 100\% & 50 & 16 \\
    \hline
    120 & 100\% & 70 & 20\\
    \hline
    160 & 100\% & 58 & 21\\
    \hline
    200 & 100\% & 52 & 21\\
    \hline
    \end{tabular}
   
    \end{center}
\end{table}

In another experiment, the nodes are made to leave the system with 10\% probability after every three minutes. For the involvement of 160 nodes, our approach achieved success rate of 99.39\% and the maximum latency of 52ms. Assuming that the human tolerance limit is about 200ms, the response is pretty good.
